Greedy Approaches to Online Stochastic Matching

Within the context of stochastic probing with commitment, we consider the online stochastic matching problem; that is, the one-sided online bipartite matching problem where edges adjacent to an online node must be probed to determine if they exist based on edge probabilities that become known when an online vertex arrives. If a probed edge exists, it must be used in the matching (if possible). We consider the competitiveness of online algorithms in both the adversarial order model (AOM) and the random order model (ROM). More specifically, we consider a bipartite stochastic graph $G = (U,V,E)$ where $U$ is the set of offline vertices, $V$ is the set of online vertices and $G$ has edge probabilities $(p_{e})_{e \in E}$ and edge weights $(w_{e})_{e \in E}$. Additionally, $G$ has probing constraints $(\scr{C}_{v})_{v \in V}$, where $\scr{C}_v$ indicates which sequences of edges adjacent to an online vertex $v$ can be probed. We assume that $U$ is known in advance, and that $\scr{C}_v$, together with the edge probabilities and weights adjacent to an online vertex are only revealed when the online vertex arrives. This model generalizes the various settings of the classical bipartite matching problem, and so our main contribution is in making progress towards understanding which classical results extend to the stochastic probing model.

==> content/conclusion-backup.tex <==
We considered the online  stochastic bipartite matching (with arbitrary patience values and offline vertex weights) problem in the random order input model (ROM). We noted how the stochastic setting generalizes the classical (i.e., non-stochastic) setting.  We introduced the non-committal benchmark, which arguably is the strongest meaningful benchmark. Our main result shows that for a broad class of stochastic graphs, we obtain a simple deterministic greedy algorithm with competitive ratio $1-\frac{1}{e} \approx 0.632$.
Currently, even for the classical (i.e., non-stochastic) setting, $1-\frac{1}{e}$ is the best ratio known for deterministic algorithms with random order input arrivals. The strongest ROM in-approximation of $0.823$ (due to Manshadi et al. \cite{ManshadiGS12}) comes from the classical i.i.d. setting for a known distribution.  

Our work leaves open many questions:
\begin{itemize}

\item Is there a provable difference between what an optimal online algorithm can obtain against 
the committal benchmark versus the non-committal benchmark? Specifically, does Algorithm \ref{alg:dynamical_program}
achieve a competitive ratio of $1-1/e$ against the non-committal benchmark which holds
for all rankable stochastic graphs or even for all stochastic graphs? 

\item What is the best ratio that a deterministic online algorithm can obtain for all stochastic graphs in the ROM setting? 
Brubach et al. achieve the optimal competitive ratio $1/2$ for adversarial input arrivals and hence the same bound holds for ROM arrivals. Can we at least make an improvement on $1/2$ which holds for all stochastic graphs?

\item Is the optimal competitive ratio for the stochastic case (for either the committal or non-committal benchmark) worse than the optimal ratio for the classical setting? Note that in the classical setting the benchmark is the weight of an offline optimal matching. 

\item Can our $1-\frac{1}{e}$ competitive ratio be improved by a randomized algorithm? Here we note that in the classical ROM setting, the Ranking algorithm achieves a $0.696$ ratio for unweighted graphs  (due to Mahdian and Yan \cite{Mahdian2011}) and a $0.6534$ ratio (due to Huang et al. \cite{huang2018online}) for vertex weighted graphs. Thus, randomization does help in the classical ROM setting. 



\end{itemize}


==> content/conclusion.tex <==
\label{sec:conclusion}
We considered the online  stochastic bipartite matching with commitment in a number of different settings establishing several compeititve bound against the optimal offline committal benchmark. In Appendix \ref{XXX} we indicate when we can use the stronger non-committal benchmark.  \ABc{Not sure which apperndices need to be referenced regarding the extsnion to the non-[committable benchmark for the special cases of rankable we provide.} 

In the case of vertex weighted stochastic graphs, adversarial input sequences, and general probing constraints, we provide a deterministic algorithm that achieves a $\frac{1}{2}$ competitive ratio. 
%against an optimal offline benchmark that respects the probing and commitment constraints. 
This is an optimal competitive ratio for deterministic algorithms and adversarial input sequences.

In the case of random order input sequences, we provide two results. First, for edge weighted stochastic graphs, and general probing constraints, we provide a randomized algorithm that achieves the optimal competitive ratio $\frac{1}{e}$. 
%against thel offline committal benchmark. 
For vertex weighted results we provide an algorithm that achieves a $1-1/e$ competitive ratio whenever the input graph is ``rankable''. Our  rankable assumption subsumes most \ABc{Is it most or all } of the  stochastic graph settings studied thus far.
% in terms of conditions on the the generality of vertex weights, edge probabilities and patience/probing  constraints. 
%
%
%
%with respect to a new stronger benchmark we define, namely an optimal offline algorithm that respects the patience constraints but does not have to respect commitment constraints.  
%This non-committal benchmark is  arguably the strongest meaningful benchmark in the stochastic probing setting. 

%%Currently, even for the classical (i.e., non-stochastic) setting, $1-\frac{1}{e}$ is the best known ratio for deterministic algorithms operating on vertex weighted graphs  with random order input arrivals. The best known ROM in-approximation $0.823$ (due to Manshadi et al. \cite{ManshadiGS12}) that comes from the classical i.i.d. unweighted graph setting for a known distribution and applies to randomized as well as deterministic algorithms. 
%
Our work leaves open many questions which we present in Appendix \ref{sec:open_problems}. 

%\begin{itemize}
%
%\item What is the best ratio that a deterministic or randomized  online algorithm  can obtain for {\it all} stochastic graphs in the ROM setting?
%That is, what competitive ratio can be achieved without the rankable assumption?
%Is there a non-trivial  probing setting (i.e. that does not reduce to the classical non-probing setting)  in which we can surpass the $1-1/e$ ``barrier''. 
%
%\item Is there a provable difference between what an optimal online algorithm can obtain against 
%the committal benchmark versus the non-committal benchmark? Specifically, does Algorithm \ref{alg:dynamical_program}
%achieve a competitive ratio of $1-1/e$ against the non-committal benchmark which holds
%for all rankable stochastic graphs or for all stochastic graphs? 
%
%\item What is the best ratio that a randomzed online algorithm can obtain for stochastic graphs in the adversarial input sequence setting? 
%Brubach et al. \cite{Brubach2019} achieve the optimal deterministic competitive ratio $1/2$ for adversarial input arrivals. Can we at least make an improvement on the $1/2$ ratio when considering randomized algorithms and adversarial input sequences? The  Mehta and Panigraphi \cite{MehtaP12} $.621$ inapproximation shows  that randomized probing algorithms (even for unweighted graphs and unit patience) cannot achieve a $1-1/e$ competitive ratio for adversarial input sequences in contrast to our results for random order input sequences. 
%
%\item Is the optimal competitive ratio for the stochastic case (for either the committal or non-committal benchmark) provably worse than the optimal ratio for the classical setting? Note that in the classical setting the benchmark is the weight of an offline optimal matching. 
%
%\item Can our $1-\frac{1}{e}$ competitive ratio be improved by a randomized algorithm? Here we note that in the classical ROM setting, the Ranking algorithm achieves a $0.696$ ratio for unweighted graphs  (due to Mahdian and Yan \cite{Mahdian2011}) and a $0.6534$ ratio (due to Huang et al. \cite{huang2018online}) for vertex weighted graphs. Thus, randomization does \AB{seem} to help in the classical ROM setting. 
%%\ABc{I phrased this as "does seem to help" as I do not know of any negative results (beyond Mandshadi) that holds for deterministic algorithms and ROM inputs. We do know that randomization helps for adversarial inputs.} 
%
%
%\end{itemize}
%%


==> content/edge_weights_proofs.tex <==
In this section, we prove Theorem \ref{thm:ROM_edge_weights}
from Section \ref{sec:edge_weights}. We first state a formal version of
\textsc{VertexProbe}:
\begin{algorithm}[H]
\caption{VertexProbe}
\label{alg:vertex_probe}
\begin{algorithmic}[1]
\Require an online vertex $s$ of a stochastic graph, $\partial(s)$, values $(z(\bm{e}))_{\bm{e} \in \scr{C}_s}$ which satisfy 
$\sum_{\bm{e} \in \scr{C}_s} z(\bm{e}) \le 1$. 
\Ensure an active edge $\scr{N}$ of $\partial(s)$.
\State $\scr{N} \leftarrow \emptyset$.
\State Return $\scr{N}$ with probability $1 - \sum_{\bm{e} \in \scr{C}_s} z(\bm{e})$
\Comment{\textit{pass} with a certain probability.} 
\State Draw $\bm{e}'$ from $\scr{C}_s$ with
probability $z(\bm{e}')$.
\State Denote $\bm{e}' = (e_{1}', \ldots ,e_{k}')$ for $k := |\bm{e}'|$.
\For{$i=1, \ldots ,k$}
\State Probe the edge $e'_i$.
\If{$\sta(e'_i)=1$}
\State  Add $e'_i$ to $\scr{N}$, and exit the ``for loop''.
\EndIf
\EndFor
\State \Return $\scr{N}$.
\end{algorithmic}
\end{algorithm}

\begin{proof}[Proof of Lemma \ref{lem:edge_value_lower_bound}]
Set $\alpha:=1/e$ for clarity, and take $t \ge \alpha n$. 
Define $e_{t}:=(u_t,v_{t})$, where $u_{t}$ is the vertex of $U$ which $v_{t}$ commits to
(which is the empty set $\emptyset$, if no such commitment occurs). 
For each $u \in U$, denote $C(u,v_t)$ as the event in which
$v_t$ commits to $u$. 
Let us now condition on the random subset $V_{t}$, as well as the 
random vertex $v_{t}$. 
In this case, 
\[
    \mb{E}[ w(e_{t})  \, | \, V_{t}, v_t] = \sum_{u \in U} w_{u,v_t} \, \mb{P}[ C(u,v_t)  \, | \, V_{t}, v_{t}].
\]
Observe however that once we condition on $V_{t}$ and $v_{t}$, Algorithm \ref{alg:ROM_edge_weights} corresponds to executing \textsc{VertexProbe} on the instance $(v_t, \partial(v_t), (x_{v_t}(\bm{e}))_{\bm{e} \in \scr{C}_v})$,
where we recall that $(x_{v}(\bm{e}))_{\bm{e} \in \scr{C}_v, v \in v_t}$ is an optimum solution
of \ref{LP:config} for $G_t=G[U \cup V_t]$. Thus,
Lemma \ref{lem:fixed_vertex_probe} implies that $\mb{P}[ C(u,v_t)  \, | \, V_{t}, v_{t}]  =  p_{u,v_t} \til{x}_{u,v_t}$,
where
\[
\til{x}_{u,v_t}:= \sum_{\substack{\bm{e}' \in \scr{C}_{v_t}: \\ e \in \bm{e}'}} g(\bm{e}_{ < e}') \cdot x_{v_t}( \bm{e}'),
\]
and so $\mb{E}[ w(e_{t})  \, | \, V_{t}, v_t] = \sum_{u \in U} w_{u,v_t}  p_{u,v_t}  \til{x}_{u,v_t}$.
On the other hand, if we condition on \textit{solely} $V_{t}$, then $v_{t}$ remains distributed uniformly
at random amongst the vertices of $V_{t}$. Moreover, once we condition on $V_t$, the graph $G_t$ is determined, and thus so are
the values $(x_{v}(\bm{e}))_{v \in V_{t}, \bm{e} \in \scr{C}_v}$. These observations together imply that
\begin{equation}\label{eqn:conditional_expectation_value}
\mb{E}[ w_{u,v_t} \, p_{u,v_t} \,  \til{x}_{u,v_t}  \, | \, V_{t}] = \frac{\sum_{v \in V_t} w_{u,v} \, p_{u,v} \, \til{x}_{u,v}}{t}
\end{equation}
for each $u \in U$ and $\alpha n \le t \le n$. If we now take expectation over $v_{t}$, then using the law of iterated
expectations,
\begin{align*}
    \mb{E}[ w(e_t)  \, | \, V_{t}] &= \mb{E}[ \,  \mb{E}[ w(e_t) \, | \, V_t, v_t] \,   \, | \, V_{t} ]  \\
                               &= \mb{E}\left[ \sum_{u \in U} w_{u,v_t} \, p_{u,v_t} \, \til{x}_{u,v_t}   \, | \, V_{t} \right] \\
                               &= \sum_{u \in U} \mb{E}[ w_{u,v_t} \, p_{u,v_t} \, \til{x}_{u,v_t}  \, | \, V_{t}] \\
                               &= \sum_{u \in U} \sum_{v \in V_t} \frac{w_{u,v} p_{u,v} \, \til{x}_{u,v}}{t},
\end{align*}
where the final equation follows from \eqref{eqn:conditional_expectation_value}.
Observe however that
\[
    \cLPOPT(G_t)=\sum_{v \in V_t} \sum_{u \in U} w_{u,v_t} \, p_{u,v_t} \, \til{x}_{u,v_t},
\]
as $(x_{v}(\bm{e}))_{v \in V_{t}, \bm{e} \in \scr{C}_v}$ is an optimum solution to
\ref{LP:config} for $G_t$. As a result,
\[
    \mb{E}[ w(e_t)  \, | \, V_{t}]  = \frac{\cLPOPT(G_t)}{t},
\]
and so
\[
	\mb{E}[ w(e_t)]  = \frac{\mb{E}[\cLPOPT(G_t)]}{t},
\]
after taking taking expectation over $V_{t}$. On the other hand, Lemma \ref{lem:random_induced_subgraph} implies that
\[
	\frac{\mb{E}[\cLPOPT(G_t)]}{t} \ge  \frac{\cLPOPT(G)}{n}.
\]
Thus,
\[
\mb{E}[ w(e_t)] \ge \frac{\cLPOPT(G)}{n},
\]
provided $ \alpha n \le t \le n$, thereby completing the proof.

\end{proof}



\begin{proof}[Proof of Lemma \ref{lem:availability_lower_bound}]
When Algorithm \ref{alg:ROM_edge_weights}
solves \ref{LP:config} for $G_t$, we notated
the variables $(\til{x}_{u,v})_{u \in U, v \in V_t}$ without
ambiguity, despite the dependence on $\alpha n \le t \le n$. For this proof, it
is necessary to be more explicit in our notation, so we denote $\til{x}_{u,v}$
as $\til{x}^{(t)}_{u,v}$ to indicate that we are working with an edge variable
from the relevant LP solution involving $G_t$. 


In what follows, let us assume that $ \alpha n \le t \le n$ is fixed. We wish to prove that for each $u \in U$, 
\[
\mb{P}[u \in R_{t}  \, | \, V_{t},v_t] \ge \frac{ \alpha n}{t-1}.
\]
As such, we must condition on $(V_t,v_t)$ throughout the remainder of the proof.
To simplify the argument, we abuse notation slightly and remove $(V_t,v_t)$
from the subsequent probability computations, though it is understood to implicitly
appear.



Given arriving node $v_{j}$ for $j=1, \ldots ,n$, once again denote $C(u,v_j)$
as the event in which $v_j$ commits to $u \in U$. As $R_{t}$ denotes the
unmatched nodes after the vertices $v_{1}, \ldots , v_{t-1}$ are processed
by Algorithm \ref{alg:ROM_edge_weights}, observe that
$u \in R_{t}$ if and only if $\neg C(u,v_j)$ occurs for each $j=1, \ldots , t-1$.
As a result,
\[
	\mb{P}[ u \in R_{t} ] = \mb{P}[\cap_{j=1}^{t-1} \neg C(u,v_j)].
\]
We therefore focus on lower bounding $\mb{P}[\cap_{j=1}^{t-1} \neg C(u,v_j) ]$ in order to prove
the lemma.

First observe that for $j=1, \ldots , \alpha n -1$, the algorithm passes on probing
$\partial(v_j)$ by definition. As such, we may focus on lower bounding
\[
	\mb{P}[\cap_{j= \alpha n}^{t-1} \neg C(u,v_j)],
\]
which depends only on the vertices of $V_{t-1} \setminus V_{\alpha n -1}$.
We denote $\bar{t}:= t - \alpha n$ as the number of vertices within this set.

Let us first consider the vertex $v_{t-1}$,
and the induced edge variable $\til{x}^{(t-1)}_{u,v}$ for each $v \in V_{t-1}$.
Observe that after applying Lemma \ref{lem:fixed_vertex_probe},
\begin{align*}
	\mb{P}[ C(u,v_{t-1})] &= \sum_{ v \in V_{t-1}} \mb{P}[ C(u,v_{t-1})  \, | \, v_{t-1} = v] \cdot \mb{P}[v_{t-1}=v] \\
											  &= \frac{1}{t-1} \sum_{v \in V_{t-1}} \til{x}_{u,v}^{(t-1)} \, p_{u,v},
\end{align*}
as once we condition on $(V_{t}, v_t)$, $v_{t-1}$ is uniformly distributed amongst $V_{t-1}$.
On the other hand, the values $(\til{x}_{u,v}^{(t-1)})_{u \in U, v \in V_{t-1}}$ are derived
from a solution to \ref{LP:config} for $G_{t-1}$, and so
\[
	\sum_{v \in V_{t-1}} \til{x}_{u,v}^{(t-1)} \, p_{u,v} \le 1.
\]
We therefore get that
\[
	\mb{P}[ C(u,v_{t-1}) ]  \le \frac{1}{t-1}.
\]
Similarly, if we fix $1 \le k \le \bar{t}$, then we can generalize the above
argument by conditioning
on the identities of all the vertices preceding $v_{t-k}$, as well as the probes
they make; that is, $(u_{t-1},v_{t-1}), \ldots ,(u_{t-(k-1)},v_{t-(k-1)})$ (in addition to $V_t$ and $v_t$ as always). 

In order to simplify the resulting indices, let us reorder the vertices of $V_{t-1} \setminus V_{\alpha n -1}$.
Specifically, define $\bar{v}_{k}:=v_{t-k}, \bar{u}_k := u_{t-k}$ and $\bar{e}_k:=e_{t-k}$
for $k=1,\ldots ,\bar{t}$. With this notation, we denote
$\scr{H}_{k}$ as encoding the information available based on the vertices $\bar{v}_1, \ldots , \bar{v}_{k}$ and the edges they (potentially) committed to, namely $\bar{e}_{1}, \ldots ,\bar{e}_{k}$\footnote{Formally, $\scr{H}_k$ is the sigma-algebra
generated from $V_t,v_t$ and $\bar{e}_{1}, \ldots ,\bar{e}_{k}$.}. By convention,
we define $\scr{H}_{0}$ as encoding the information regarding $V_t$ and $v_t$. 

An analogous computation to the above case then implies that
\[
	\mb{P}[ C(u,\bar{v}_{k})  \, | \, \scr{H}_{k-1}] = \sum_{ v \in V_{t-k}} \til{x}_{u,v}^{(t-k)} \, p_{u,v} \, \mb{P}[\bar{v}_k=v] \le \frac{1}{t-k},
\]
for each $k=1,\ldots , \bar{t}$, where
$\til{x}_{u,v}^{(t-k)}$ is the edge variable for $v \in V_{t-k}$.

Observe now that in each step, we condition on strictly more information;
that is, $\scr{H}_{k-1} \subseteq \scr{H}_{k}$
for each $k=2, \ldots , \bar{t}$. On the other hand, observe that
if we condition on $\scr{H}_{k-1}$ for $1 \le k \le \bar{t}-1$,
then the event $C(u,\bar{v}_{j})$ can be determined from $\scr{H}_{k-1}$
for each $1 \le j \le k-1$.



Using these observations, for $1 \le k \le \bar{t}$, the following recursion holds:
\begin{align*}
\mb{P}[ \cap_{j=1}^{k} \neg C(u,\bar{v}_j)] 
  &= \mb{E}\left[ \, \mb{E}\left[ \prod_{j=1}^{k} \bm{1}_{ [\neg C(u,\bar{v}_j)]}  \, | \, \scr{H}_{k-1}\right] \right]	\\
&= \mb{E}\left[ \,  \prod_{j=1}^{k-1} \bm{1}_{ [\neg C(u,\bar{v}_j)]} \, \mb{P}[\neg C(\bar{v}_k, u)  \, | \, \scr{H}_{k-1}]\right] \\
&\ge \left(1 - \frac{1}{t-k}\right) \mb{P}[ \cap_{j=1}^{k-1} \neg C(u,\bar{v}_j)]
\end{align*}
It follows that if $k= t - \alpha n$, then applying the above recursion implies that
\[
	\mb{P}[\cap_{j= \alpha n}^{t-1} \neg C(u,v_j)] \ge \prod_{k=1}^{t- \alpha n} \left(1 - \frac{1}{t-k}\right).
\]
Thus, after cancelling the pairwise products,
\[
	 \mb{P}[\cap_{j= \alpha n}^{t-1}\neg C(u,v_j)] \ge  \frac{\alpha n}{t-1},
\]
and so 
\[
		\mb{P}[ u \in R_{t}] = \mb{P}[\cap_{j= \alpha n}^{t-1}\neg C(u,v_j)] \ge \frac{\alpha n}{t-1}
\]
thereby completing the argument.


\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:ROM_edge_weights}]
Clearly, Algorithm \ref{alg:ROM_edge_weights} can be implemented efficiently, since \ref{LP:config} is efficiently solvable,
provided it involves a stochastic graph whose probing constraints are permutation-closed.
Thus, we focus on proving the algorithm attains the desired asymptotic competitive ratio.


Let us consider the matching $\scr{M}$ returned by the algorithm,
as well as its weight, which we denote by $w(\scr{M})$. Set $\alpha:=1/e$ for clarity, and take $t \ge \alpha n$. For each $\alpha n \le t \le n$, define $R_{t}$ as the \textit{unmatched vertices} of $U$ when vertex $v_{t}$ arrives. Moreover, define $e_{t}$
as the edge $v_{t}$ commits to, which is $\emptyset$ if no such commitment
is made. Observe that
\begin{equation}\label{eqn:value_of_matching}
   \mb{E}[ w(\scr{M}) ] = \sum_{t=\alpha n}^{n} \mb{E}[ w(u_t, v_t) \cdot \bm{1}_{[u_t \in R_t]} ].
\end{equation}
Fix $\alpha n \le t \le n$, and first observe that $w(u_t, v_t)$ and $\{ u_{t} \in R_t \}$ are conditionally independent given
$(V_{t},v_t)$, as the probes involving $\partial(v_t)$ are independent from those of $v_{1}, \ldots ,v_{t-1}$. Thus,
\[
\mb{E}[ w(u_t,v_t) \cdot \bm{1}_{[u_t \in R_t]}  \, | \, V_{t}, v_{t}] = \mb{E}[ w(u_t,v_t)  \, | \, V_t, v_t] \cdot \mb{P}[ u_t \in R_t  \, | \, V_{t}, v_t].
\]
Moreover, Lemma \ref{lem:availability_lower_bound} implies that
\[    
   \mb{E}[ w(u_t,v_t)  \, | \, V_t, v_t] \cdot \mb{P}[ u_t \in R_t  \, | \, V_{t}, v_t] \ge 
   \mb{E}[ w(u_t,v_t)  \, | \, V_{t}, v_t] f(t,n),
\]
and so $\mb{E}[ w(u_t,v_t) \, \bm{1}_{[u_t \in R_t]}  \, | \, V_{t}, v_{t}] \ge \mb{E}[ w(u_t,v_t)  \, | \, V_{t}, v_t] \, f(t,n)$.
Thus, by the law of iterated expectations\footnote{$\mb{E}[ w(u_t,v_t) \cdot \bm{1}_{[u_t \in R_t]}  \, | \, V_{t}, v_{t}]$
is a random variable which depends on $V_t$ and $v_t$, and so the outer expectation is over the randomness in $V_t$ and $v_t$.}
\begin{align*}
\mb{E}[ w(u_t,v_t) \cdot \bm{1}_{[u_t \in R_t]} ] &= \mb{E}[ \, \mb{E}[ w(u_t,v_t) \cdot \bm{1}_{[u_t \in R_t]}  \, | \, V_{t}, v_{t}] \, ] \\
			&\ge \mb{E}[ \, \mb{E}[ w(u_t,v_t)  \, | \, V_{t}, v_t]  f(t,n) \, ] 
			= f(t,n) \mb{E}[ w(u_t,v_t)].
\end{align*}
As a result, using \eqref{eqn:value_of_matching}, we get that
\begin{align*}
	\mb{E}[w(\scr{M})] &= \sum_{t=\alpha n}^{n} \mb{E}[ w(u_t, v_t) \, \bm{1}_{[u_t \in R_t]} ]
						  \ge \sum_{t=\alpha n}^{n} f(t,n) \, \mb{E}[ w(u_t,v_t)].
\end{align*}
We may thus conclude that
\[
    \mb{E}[ w(\scr{M})] \ge \LPOPT_{conf}(G) \sum_{t=\alpha n}^{n} \frac{ f(t,n)}{n},
\]
after applying Lemma \ref{lem:edge_value_lower_bound}. 
As $\sum_{t=\alpha n}^{n} f(t,n)/n \ge (1/e -1/|V|)$, the result holds.


\end{proof}










==> content/non_committal_negative.tex <==

\begin{proposition}\label{prop:negative_online_node}
There exists a stochastic graph $G$ with a single online node, such
that $\OPT(G) = 0.856269 \cdot \nOPT(G)$. 
\end{proposition}
\begin{proof}[Proof of Proposition \ref{prop:negative_online_node}]
Suppose $G$ has a single online node $v$ with patience $\ell_{v} =2$, and that there are $3$ offline nodes $U=\{u_{1}, u_{2}, u_{3}\}$. For each $i \in \{1,2,3\}$, we denote the weight of $(u_{i},v)$ by $w_{i}$ and assume that the edge $(u_i,v)$
is active with probability $p_{i}$. We make the following assumptions on these weights
and probabilities:
\begin{enumerate}
\item $w_{1} < w_{2} < w_{3}$.
\item $p_{1} > p_{2} > p_{3}$.
\item $w_{1} \cdot p_{1} \ge w_{2} \cdot p_{2} > w_{3} \cdot p_{3}$. \label{eqn:expected_reward}
\item $p_{2} \cdot w_{2} - p_{3} \cdot w_{3} \ge p_{1} \cdot w_{1} \cdot (p_{2} - p_{3})$ \label{eqn:OPT_strategy}
\end{enumerate}
Clearly, there exists a choice of weights and probabilities which satisfy these constraints. For instance,
take $w_{1} =3$, $w_{2} =4$, $w_{3}= 98$, $p_{1}=0.8$, $p_{2}=0.6$, and $p_{3} =0.01$.
Based on these assumptions let us now consider the value of $\OPT(G)$. Observe that
\[
	p_{2} \cdot w_{2} + (1 - p_{2}) \cdot p_{1} \cdot w_{1} \ge p_{3} \cdot w_{3} + (1- p_{3}) \cdot p_{1} \cdot w_{1}
															\ge p_{3} \cdot w_{3} + (1 - p_{3}) \cdot p_{2} \cdot w_{2},
\]
where the first inequality follows from \eqref{eqn:OPT_strategy}, and the second follows from \eqref{eqn:expected_reward}.
As a result, it is clear to see that the committal benchmark corresponds to probing $u_{2}$ and then $u_{1}$ (if necessary);
thus, $\OPT(G) = p_{2} \cdot w_{2} + (1 - p_{2}) \cdot p_{1} \cdot w_{1}$.

On the other hand, let us consider $\nOPT(G)$, the value of the non-committal benchmark on $G$.
Consider the following \textit{non-committal} probing algorithm:
\begin{itemize}
\item Probe $(u_{2},v)$, and if $\sta(u_{2},v)=1$, probe $(u_{3},v)$. \label{eqn:adaptive_step}
\item Else if $\sta(u_{2},v)=0$, probe $(u_{1},v)$.
\item Return the edge of highest weight which is active (if any).
\end{itemize}

Clearly, this probing algorithm uses adaptivity to decide whether to reveal $(u_{3},v)$ or
$(u_{1},v)$ in its second probe. Specifically, if it discovers that $(u_{2},v)$ is active,
then it knows that it will return an edge with weight at least $w_{2}$. As such, it only
makes sense for $(u_{3},v)$ to be its next probe, as $w_{3} > w_{2} > w_{1}$.
On the other hand, if $(u_{2},v)$ is discovered to be inactive, it makes sense to
prioritize probing the edge $(u_{1},v)$ over $(u_{3},v)$, as the \textit{expected}
reward is higher; namely, $w_{1} \cdot p_{1} > w_{3} \cdot p_{3}$.
Thus, it is clear that the expected weight of the edge returned is 
\[
p_{2} \cdot p_{3} \cdot w_{3} + p_{2} \cdot (1 - p_{3}) \cdot w_{2} + (1 - p_{2}) \cdot p_{1} \cdot w_{1}.
\] 
Observe however that
\begin{align*}
	p_{2} \cdot p_{3} \cdot w_{3} + p_{2} \cdot (1 - p_{3}) \cdot w_{2} + (1 - p_{2}) \cdot p_{1} \cdot w_{1} 
				  &> p_{2} \cdot w_{2} + (1 - p_{2}) \cdot p_{1} \cdot w_{1}	\\
				  &= \OPT(G),
\end{align*}
where the final inequality follows since $w_{3} > w_{2}$.
As a result, it is clear that this strategy corresponds to the non-committal benchmark, and so 
$\OPT_{non}(G) > \OPT(G)$. In fact,
for the specific choice when $w_{1} =3$, $w_{2} =4$, $w_{3}= 98$, $p_{1}=0.8$, $p_{2}=0.6$, and $p_{3} =0.01$,
it holds that
\[
 	\frac{\OPT(G)}{\nOPT(G)} = 0.856269. 
\]
\end{proof}
This example slightly improves upon the negative result of \cite{costello2012matching}, in which Costello et al. show
that the ratio between $\OPT(G)$ and $\OPT_{non}(G)$ is at most $0.898$ (albeit for unweighted graphs).  

We remark that restricted to a single online node, the non-committal probing problem is a special case of
the \textit{adaptive} version \textsc{ProblemMax}, a stochastic probing problem which is studied in \cite{Asadpour2016, Fu2018, Segev2020}. Similarly, the committal probing problem is a special case of the \textit{non-adaptive} version of
\textsc{ProblemMax}, which is also considered in \cite{Asadpour2016, Fu2018, Segev2020}. Thus, we can view $0.856269$
as an upper bound (negative result) on the \textbf{adaptivity gap} of \textsc{ProblemMax}. This is in contrast to the
lower bound of $1-1/e$ on the adaptivity gap of \textsc{ProblemMax} proven by Asadpour et al. \cite{Asadpour2016}. 


%&= p_{2} \cdot w_{2} \cdot ( (1- p_{3}) + p_{3} \cdot w_{3}/ w_{2}) + (1- p_{2}) \cdot p_{1} \cdot w_{1}	\\



==> content/old_files/preliminaries.tex <==
\subsection{Preliminaries}


An input to the \textbf{online stochastic matching problem} is a \textbf{(bipartite) stochastic graph}, specified in the following way. Let $G=(U,V,E)$ be a bipartite graph with edge weights $(w_{e})_{e \in E}$ and edge probabilities $(p_{e})_{e \in E}$.
We draw an independent Bernoulli random variable of parameter $p_{e}$
for each $e \in E$. We refer to this Bernoulli as the \textbf{state} of the edge $e$, and 
denote it by $\sta(e)$. If $\sta(e)=1$, then we say that $e$ is \textbf{active}, and otherwise we say that
$e$ is \textbf{inactive}. For each $v \in V$, suppose that $\partial(v)^{(*)}$ corresponds to the collection of strings (tuples) formed from \textit{distinct} edges of $\partial(v)$. Each $v \in V$ has an \textbf{online probing constraint} $\scr{C}_v \subseteq \partial(v)^{(*)}$ which is \textbf{prefix-closed}.
That is, $\scr{C}_v$ has the property that if $\bm{e} \in \scr{C}_v$,
then so is any prefix string of $\bm{e}$. Thus, in particular,
this setting encodes the case when $v$ has a patience value $\ell_v$, and more generally, when $\scr{C}_v$
corresponds to a matroid or budgetary constraint on $\partial(v)$.
In order to discuss the efficiency of an online probing algorithm in this model,
we work in the \textbf{membership query model}.
That is, upon receiving the online vertex $v \in V$,
an online probing algorithm may make a \textbf{membership query} to any string $\bm{e} \in \partial(v)^{(*)}$,
thus determining in a single operation whether 
or not $\bm{e} \in \partial(v)^{(*)}$ is in $\scr{C}_v$. 

A solution to the online stochastic matching problem is an \textbf{online probing algorithm}. An online probing algorithm
is initially only aware of the offline vertices $U$ of $G$. We think of $V$, as well as the relevant edges probabilities, weights,
and probing constraints. as being generated by an adversary. An ordering on $V$ is then generated either through an adversarial process or uniformly at random. We refer to the
former case as the \textbf{adversarial setting} and the latter case as the \textbf{ROM setting}.

Based on whichever ordering is generated on $V$,
the nodes are then presented to the online probing algorithm one by one.
When an online node $v \in V$ arrives, the online probing algorithm sees all the adjacent edges and their associated probabilities,
as well as $\scr{C}_v$. However, the edge states $(\sta(e))_{e \in \partial(v)}$
remain hidden to the algorithm. Instead, the algorithm must perform a \textbf{probing operation} on an adjacent edge $e$ to reveal/expose its state, $\sta(e)$. In fact, the online probing algorithm must \textbf{respect commitment}.
That is, if an edge $e = (u,v)$ is probed and turns out to be active, then $e$ must be added to the current matching, provided $u$ and $v$ are both currently unmatched. The probing constraint $\scr{C}_v$ of the online node then restricts
which sequences of probes can be made to $\partial(v)$. As in the classical problem, an online probing algorithm must decide on a possible match for an online node $v$ before seeing the next online node. The goal of the online probing algorithm 
is to return a matching whose expected weight is as large as possible.

It is easy to see we cannot hope to obtain a non-trivial
competitive ratio against the expected value of an optimum matching of the stochastic graph\footnote{Consider a single online vertex with patience $1$, and $n$ offline (unweighted) vertices where each edge $e$ has probability $\frac{1}{n}$ of being present. The expectation of an online probing algorithm will be at most $\frac{1}{n}$ while the expected size of an optimal matching (over all instantiations of the edge probabilities) will be $1 - (1-\frac{1}{n})^n \rightarrow 1 -\frac{1}{e}$. This example clearly shows that no constant ratio is possible if the patience is sublinear (in $n = |U|$).}.  
Thus, the standard is the literature is to instead benchmark the performance of an online
probing algorithm against an \textit{optimum offline probing algorithm}. An \textbf{offline probing algorithm}
knows $G=(U,V,E)$ upfront, but initially the edge states $(\sta(e))_{e \in E}$ are hidden. It can adaptively probe the edges of $E$ in any order, but must satisfy the probing constraints $(\scr{C}_v)_{v \in V}$ at each step of its execution,
while respecting commitment -- that is, if a probed edge $e=(u,v)$ turns out to be active,
then $e$ is added to the matching (if possible). The goal of an offline probing
algorithm is to build a matching whose weight is as large as possible in expectation. We define
the \textbf{committal benchmark} on $G$ as an offline probing algorithm which returns
a matching whose expected weight is best possible, and denote this value by $\OPT(G)$.

We also introduce another benchmark which we refer to as the \textbf{non-committal benchmark}.
This benchmark must still adaptively probe edges subject to probing constraints, and its goal
is the same as before, but it does not need to respect
commitment. More precisely, if $P_a \subseteq E$ corresponds to
the active probes made by the benchmark, then
it returns a matching $\scr{M} \subseteq P_a$ of maximum weight.
We denote $\OPT_{non}(G)$ as the expected value of the matching that the non-committal benchmark constructs. Observe that in the case of \textbf{full patience} (i.e., $\ell_{v} = |U|$ for all $v \in V$), the benchmark may probe all the edges of $G$,
and thus corresponds to the expected weight of the optimum matching of the stochastic graph.
Clearly the non-committal benchmark is no weaker than the committal benchmark;
that is, $\OPT_{non}(G) \ge \OPT(G)$ for any stochastic graph $G$. 


Let $G =(U,V,E)$ be a stochastic graph, and fix $S \subseteq U \sqcup V$.
We define the \textbf{induced stochastic subgraph},
denoted $G[S]$, which corresponds to restricting the stochastic
graph $G$ to the vertices $S$, and retaining the relevant edge probabilities,
edge weights and probing constraint of $G$.























\subsection{Our Results}


We first consider the unknown stochastic matching problem in
the most general setting of arbitrary edge weights, and prefix-closed probing constraints.
Note that since no non-trivial competitive ratio can be proven in the case of adversarial
arrivals, we work in the ROM setting.


\begin{theorem}\label{thm:ROM_edge_weights}
Suppose the adversary presents an edge-weighted stochastic graph $G=(U,V,E)$, 
with prefix-closed probing constraints $(\scr{C}_v)_{v \in V}$. If $\scr{M}$
is the matching returned by Algorithm \ref{alg:ROM_edge_weights} when executing on $G$,
then 
\[
	\mb{E}[w(\scr{M})] \ge \left(\frac{1}{e} - \frac{1}{|V|} \right) \cdot \OPT(G),
\]
provided the vertices of $V$ arrive $u.a.r.$.

\end{theorem}
Algorithm \ref{alg:ROM_edge_weights} can be viewed as a generalization of the matching algorithm of Kesselheim et al. \cite{KRTV2013}, as our algorithm attains the optimum asymptotic competitive ratio of $1/e$.

We say that $\scr{C}_v$ is \textbf{permutation-closed}, provided if $\bm{e} \in \scr{C}_v$,
then so is any permutation string of $\bm{e}$. Observe that if $\scr{C}_v$
is both prefix-closed and permutation-closed, then it corresponds to a downward closed
set system on $\partial(v)$. 


\begin{theorem}\label{thm:ROM_edge_weights_efficiency}
If the constraints $(\scr{C}_v)_{v \in V}$
are prefix-closed and permutation-closed, then Algorithm \ref{alg:ROM_edge_weights}
can be implemented efficiently in the membership oracle model.
\end{theorem}




\subsubsection{Vertex Weights}

Since Theorem \ref{thm:ROM_edge_weights} achieves an optimum competitive ratio in
for edge weights, in order to improve upon
the ratio of $1/e$, we consider the case when the stochastic
graph $G=(U,V,E)$ has \textbf{(offline) vertex weights} -- that
is, there exists $(w_u)_{u \in U}$ such that $w_{u,v} = w_{u}$ for each $v \in N(u)$.



In the presence of vertex weights,
we consider a \textit{greedy} online probing algorithm.
That is, upon the arrival of $v$
the probes to $\partial(v)$
are made in such a way that $v$ gains as much value
as possible (in expectation), provided the currently unmatched nodes of $U$
are equal to $R$. As such, we must follow the probing strategy
of the committal benchmark when restricted to $G[ \{v\} \cup R]$,
which we denote by $\OPT(v,R)$ for convenience.


Observe that if $v$ has unit
patience, $\OPT(v,R)$  reduces to probing the edge $(u,v) \in R \times \{v\}$ such that
the value $w_{u} \cdot p_{u,v}$ is maximized. Moreover, 
$v$ has full patience, $\OPT(v,R)$ corresponds to probing
the edges of $R \times \{v\}$ in non-increasing order of the associated vertex weights. 
Brubach et al. \cite{Brubach2019} showed how to devise an \textit{efficient} probing strategy for $v$ whose expected value matches $\OPT(v,R)$, no matter the patience constraint. Using this probing strategy,
they devised an online probing algorithm which achieves a competitive ratio of $1/2$, for arbitrary 
patience values. We extend their work to handle the case of general probing
constraints $(\scr{C}_v)_{v \in V}$.


\begin{theorem}
Suppose the adversary presents a vertex weighted stochastic graph $G=(U,V,E)$, 
with prefix-closed probing constraints $(\scr{C}_v)_{v \in V}$. If $\scr{M}$
is the matching returned by Algorithm \ref{alg:dynamical_program} when executing on $G$,
then 
\[
	\mb{E}[w(\scr{M})] \ge \frac{1}{2} \cdot \OPT(G),
\]
provided the vertices of $V$ arrive in adversarial order. Moreover, Algorithm \ref{alg:ROM_edge_weights}
can be implemented efficiently, provided the constraints $(\scr{C}_v)_{v \in V}$ are permutation-closed.
\end{theorem}


Since Algorithm \ref{alg:dynamical_program} is deterministic, the $1/2$ competitive ratio
is best possible in the adversarial input setting. Thus, we next consider the same
algorithm in the ROM setting. 

Unlike the adversarial setting, the complexity of the constraints
$(\scr{C}_v)_{ v\in V}$ greatly impacts what we are able to prove.
We first start with the simplest setting in which each online vertex $v \in V$ has unit patience. Upon
the arrival of vertex $v$, Algorithm \ref{alg:dynamical_program} reduces
to probing the edge $e =(u,v) \in \partial(v)$ such that $u \in U$ is currently unmatched,
and for which $w_{u} \cdot p_{u,v}$ is
maximized. Let us refer to this online probing algorithm as \textsc{GreedyProbe}. 


\begin{theorem} \label{cor:ROM_greedy_unit}
\textsc{GreedyProbe} is a deterministic online probing algorithm
which achieves a competitive ratio of $1 - 1/e$ against
the non-committal benchmark in the ROM setting
with unit patience values, arbitrary edge probabilities and offline vertex weights.
\end{theorem}
We remark that the analysis of Theorem \ref{thm:ROM_greedy_unit} is tight since an execution of \textsc{GreedyProbe} corresponds to the seminal Karp et al. \cite{KarpVV90} Ranking algorithm for unweighted non-stochastic (i.e., $p_{u,v} \in \{0,1\}$ for all $(u,v)\in U \times V$) bipartite  matching. More precisely, in the classical (unweighted, non-stochastic) online matching problem, an execution of the randomized Ranking algorithm in the adversarial setting can be coupled with an execution of the deterministic greedy algorithm in the ROM setting -- the latter of which is a special case of \textsc{GreedyProbe}. The tightness of the ratio $1-1/e$ therefore follows since this ratio is tight for the Ranking algorithm. 


In order to prove Theorem \ref{thm:ROM_greedy_unit}, we consider an LP originally introduced in \cite{BansalGLMNR12, MehtaP12}, specialized to the case in which the stochastic graph $G$ has unit patience and offline vertex weights. 
\begin{align} \label{LP:standard_benchmark}
\tag{LP-std}
&\text{maximize}&  \sum_{u \in U, v \in V} w_u \cdot p_{u, v} \cdot x_{u, v}\\
&\text{subject to}& \sum_{v \in V} p_{u, v} \cdot x_{u,v} &\leq 1 && \forall u \in U\\
&&\sum_{u \in U} x_{u, v} &\leq 1 && \forall v \in V\\
&&  x_{u, v}  &\ge 0 && \forall u \in U, v \in V
\end{align}
If we denote $\LPOPT_{std}(G)$ as the value of an optimum solution to this LP,
then it was shown in \cite{BansalGLMNR12, MehtaP12} that \ref{LP:standard_benchmark}
is a \textbf{relaxation of the committal benchmark}; that is, $\OPT(G) \le \LPOPT_{std}(G)$.
We prove Theorem \ref{thm:ROM_greedy_unit} by first comparing the performance of \textsc{GreedyProbe} to $\LPOPT_{std}(G)$,
and then arguing that \ref{LP:standard_benchmark} is in fact a \textbf{relaxation of the non-committal benchmark};
that is $\OPT_{non}(G) \le \LPOPT_{std}(G)$.


Interestingly, Mehta and Panigraphi \cite{MehtaP12} showed that $.621 < 1-\frac{1}{e}$ is a randomized in-approximation in regard to  guarantees made against \ref{LP:standard_benchmark} in the adversarial input model with unit patience.
Theorem \ref{thm:ROM_greedy_unit} implies that this in-approximation does \textit{not} apply to the setting of ROM arrivals,
even for deterministic probing algorithms.





%Consider the natural generalization of \textsc{GreedyProbe}, based on the paradigm that when $v \in V$ arrives, the top $\ell_{v}$
%edges of $\partial(v)$ are probed in non-increasing order, based on the values $(w_{u} \, p_{u,v})_{(u,v) \in U}$
%and the availability of corresponding offline vertices. It was shown in \cite{Brubach2019} that no non-trivial competitive ratio can be proven for \textsc{GreedyProbes}, which holds for \textit{all} vertex-weighted stochastic graph
%instances. To see this, observe that for a fixed online vertex $v \in V$, the performance
%of \textsc{GreedyProbes} on $G[\{v\} \cup U]$ may be a factor $\Theta(\ell_v)$
%smaller than $\OPT(v,U,\ell_v)$.

\begin{theorem}\label{thm:greedy_probes}

Suppose Algorithm \ref{alg:dynamical_program} returns the matching $\scr{M}$ when
executing on the vertex-weighted stochastic graph $G=(U,V,E)$. 
In this case, 
\[
	\mb{E}[ w(\scr{M}) ] \ge  \left(1 - \frac{1}{e} \right) \cdot \OPT_{non}(G),
\]
provided the vertices of $V$ arrive $u.a.r.$.

\end{theorem}














==> content/old_files/results.tex <==
We first consider the unknown stochastic matching problem in
the most general setting of arbitrary edge weights, and prefix-closed probing constraints.
Note that since no non-trivial competitive ratio can be proven in the case of adversarial
arrivals, we work in the ROM setting.


\begin{theorem}\label{thm:ROM_edge_weights}
Suppose the adversary presents an edge-weighted stochastic graph $G=(U,V,E)$, 
with prefix-closed probing constraints $(\scr{C}_v)_{v \in V}$. If $\scr{M}$
is the matching returned by Algorithm \ref{alg:ROM_edge_weights} when executing on $G$,
then 
\[
	\mb{E}[w(\scr{M})] \ge \left(\frac{1}{e} - \frac{1}{|V|} \right) \cdot \OPT(G),
\]
provided the vertices of $V$ arrive $u.a.r.$.

\end{theorem}
Algorithm \ref{alg:ROM_edge_weights} can be viewed as a generalization of the matching algorithm of Kesselheim et al. \cite{KRTV2013}, as our algorithm attains the optimum asymptotic competitive ratio of $1/e$.

We say that $\scr{C}_v$ is \textbf{permutation-closed}, provided if $\bm{e} \in \scr{C}_v$,
then so is any permutation string of $\bm{e}$. Observe that if $\scr{C}_v$
is both prefix-closed and permutation-closed, then it corresponds to a downward closed
set system on $\partial(v)$. 


\begin{theorem}\label{thm:ROM_edge_weights_efficiency}
If the constraints $(\scr{C}_v)_{v \in V}$
are prefix-closed and permutation-closed, then Algorithm \ref{alg:ROM_edge_weights}
can be implemented efficiently in the membership oracle model.
\end{theorem}




\subsubsection{Vertex Weights}

Since Theorem \ref{thm:ROM_edge_weights} achieves an optimum competitive ratio in
for edge weights, in order to improve upon
the ratio of $1/e$, we consider the case when the stochastic
graph $G=(U,V,E)$ has \textbf{(offline) vertex weights} -- that
is, there exists $(w_u)_{u \in U}$ such that $w_{u,v} = w_{u}$ for each $v \in N(u)$.



In the presence of vertex weights,
we consider a \textit{greedy} online probing algorithm.
That is, upon the arrival of $v$
the probes to $\partial(v)$
are made in such a way that $v$ gains as much value
as possible (in expectation), provided the currently unmatched nodes of $U$
are equal to $R$. As such, we must follow the probing strategy
of the committal benchmark when restricted to $G[ \{v\} \cup R]$,
which we denote by $\OPT(v,R)$ for convenience.


Observe that if $v$ has unit
patience, $\OPT(v,R)$  reduces to probing the edge $(u,v) \in R \times \{v\}$ such that
the value $w_{u} \cdot p_{u,v}$ is maximized. Moreover, 
$v$ has full patience, $\OPT(v,R)$ corresponds to probing
the edges of $R \times \{v\}$ in non-increasing order of the associated vertex weights. 
Brubach et al. \cite{Brubach2019} showed how to devise an \textit{efficient} probing strategy for $v$ whose expected value matches $\OPT(v,R)$, no matter the patience constraint. Using this probing strategy,
they devised an online probing algorithm which achieves a competitive ratio of $1/2$, for arbitrary 
patience values. We extend their work to handle the case of general probing
constraints $(\scr{C}_v)_{v \in V}$.


\begin{theorem}
Suppose the adversary presents a vertex weighted stochastic graph $G=(U,V,E)$, 
with prefix-closed probing constraints $(\scr{C}_v)_{v \in V}$. If $\scr{M}$
is the matching returned by Algorithm \ref{alg:dynamical_program} when executing on $G$,
then 
\[
	\mb{E}[w(\scr{M})] \ge \frac{1}{2} \cdot \OPT(G),
\]
provided the vertices of $V$ arrive in adversarial order. Moreover, Algorithm \ref{alg:ROM_edge_weights}
can be implemented efficiently, provided the constraints $(\scr{C}_v)_{v \in V}$ are permutation-closed.
\end{theorem}


Since Algorithm \ref{alg:dynamical_program} is deterministic, the $1/2$ competitive ratio
is best possible in the adversarial input setting. Thus, we next consider the same
algorithm in the ROM setting. 

Unlike the adversarial setting, the complexity of the constraints
$(\scr{C}_v)_{ v\in V}$ greatly impacts what we are able to prove.
We first start with the simplest setting in which each online vertex $v \in V$ has unit patience. Upon
the arrival of vertex $v$, Algorithm \ref{alg:dynamical_program} reduces
to probing the edge $e =(u,v) \in \partial(v)$ such that $u \in U$ is currently unmatched,
and for which $w_{u} \cdot p_{u,v}$ is
maximized. Let us refer to this online probing algorithm as \textsc{GreedyProbe}. 


\begin{theorem} \label{cor:ROM_greedy_unit}
\textsc{GreedyProbe} is a deterministic online probing algorithm
which achieves a competitive ratio of $1 - 1/e$ against
the non-committal benchmark in the ROM setting
with unit patience values, arbitrary edge probabilities and offline vertex weights.
\end{theorem}
We remark that the analysis of Theorem \ref{thm:ROM_greedy_unit} is tight since an execution of \textsc{GreedyProbe} corresponds to the seminal Karp et al. \cite{KarpVV90} Ranking algorithm for unweighted non-stochastic (i.e., $p_{u,v} \in \{0,1\}$ for all $(u,v)\in U \times V$) bipartite  matching. More precisely, in the classical (unweighted, non-stochastic) online matching problem, an execution of the randomized Ranking algorithm in the adversarial setting can be coupled with an execution of the deterministic greedy algorithm in the ROM setting -- the latter of which is a special case of \textsc{GreedyProbe}. The tightness of the ratio $1-1/e$ therefore follows since this ratio is tight for the Ranking algorithm. 


In order to prove Theorem \ref{thm:ROM_greedy_unit}, we consider an LP originally introduced in \cite{BansalGLMNR12, MehtaP12}, specialized to the case in which the stochastic graph $G$ has unit patience and offline vertex weights. 
\begin{align} \label{LP:standard_benchmark}
\tag{LP-std}
&\text{maximize}&  \sum_{u \in U, v \in V} w_u \cdot p_{u, v} \cdot x_{u, v}\\
&\text{subject to}& \sum_{v \in V} p_{u, v} \cdot x_{u,v} &\leq 1 && \forall u \in U\\
&&\sum_{u \in U} x_{u, v} &\leq 1 && \forall v \in V\\
&&  x_{u, v}  &\ge 0 && \forall u \in U, v \in V
\end{align}
If we denote $\LPOPT_{std}(G)$ as the value of an optimum solution to this LP,
then it was shown in \cite{BansalGLMNR12, MehtaP12} that \ref{LP:standard_benchmark}
is a \textbf{relaxation of the committal benchmark}; that is, $\OPT(G) \le \LPOPT_{std}(G)$.
We prove Theorem \ref{thm:ROM_greedy_unit} by first comparing the performance of \textsc{GreedyProbe} to $\LPOPT_{std}(G)$,
and then arguing that \ref{LP:standard_benchmark} is in fact a \textbf{relaxation of the non-committal benchmark};
that is $\OPT_{non}(G) \le \LPOPT_{std}(G)$.


Interestingly, Mehta and Panigraphi \cite{MehtaP12} showed that $.621 < 1-\frac{1}{e}$ is a randomized in-approximation in regard to  guarantees made against \ref{LP:standard_benchmark} in the adversarial input model with unit patience.
Theorem \ref{thm:ROM_greedy_unit} implies that this in-approximation does \textit{not} apply to the setting of ROM arrivals,
even for deterministic probing algorithms.





%Consider the natural generalization of \textsc{GreedyProbe}, based on the paradigm that when $v \in V$ arrives, the top $\ell_{v}$
%edges of $\partial(v)$ are probed in non-increasing order, based on the values $(w_{u} \, p_{u,v})_{(u,v) \in U}$
%and the availability of corresponding offline vertices. It was shown in \cite{Brubach2019} that no non-trivial competitive ratio can be proven for \textsc{GreedyProbes}, which holds for \textit{all} vertex-weighted stochastic graph
%instances. To see this, observe that for a fixed online vertex $v \in V$, the performance
%of \textsc{GreedyProbes} on $G[\{v\} \cup U]$ may be a factor $\Theta(\ell_v)$
%smaller than $\OPT(v,U,\ell_v)$.

\begin{theorem}\label{thm:greedy_probes}

Suppose Algorithm \ref{alg:dynamical_program} returns the matching $\scr{M}$ when
executing on the vertex-weighted stochastic graph $G=(U,V,E)$. 
In this case, 
\[
	\mb{E}[ w(\scr{M}) ] \ge  \left(1 - \frac{1}{e} \right) \cdot \OPT_{non}(G),
\]
provided the vertices of $V$ arrive $u.a.r.$.

\end{theorem}











==> content/open-problems <==

\begin{itemize}

\item What is the best ratio that a deterministic or randomized  online algorithm  can obtain for {\it all} stochastic graphs in the ROM setting?
That is, what competitive ratio can be achieved without the rankable assumption?
Is there a non-trivial  probing setting (i.e. that does not reduce to the classical non-probing setting)  in which we can surpass the $1-1/e$ ``barrier''. 

\item Is there a provable difference between what an optimal online algorithm can obtain against 
the committal benchmark versus the non-committal benchmark? Specifically, does Algorithm \ref{alg:dynamical_program}
achieve a competitive ratio of $1-1/e$ against the non-committal benchmark which holds
for all rankable stochastic graphs or for all stochastic graphs? 

\item What is the best ratio that a randomzed online algorithm can obtain for stochastic graphs in the adversarial input sequence setting? 
Brubach et al. \cite{Brubach2019} achieve the optimal deterministic competitive ratio $1/2$ for adversarial input arrivals. Can we at least make an improvement on the $1/2$ ratio when considering randomized algorithms and adversarial input sequences? The  Mehta and Panigraphi \cite{MehtaP12} $.621$ inapproximation shows  that randomized probing algorithms (even for unweighted graphs and unit patience) cannot achieve a $1-1/e$ competitive ratio for adversarial input sequences in contrast to our results for random order input sequences. 

\item Is the optimal competitive ratio for the stochastic case (for either the committal or non-committal benchmark) provably worse than the optimal ratio for the classical setting? Note that in the classical setting the benchmark is the weight of an offline optimal matching. 

\item Can our $1-\frac{1}{e}$ competitive ratio be improved by a randomized algorithm? Here we note that in the classical ROM setting, the Ranking algorithm achieves a $0.696$ ratio for unweighted graphs  (due to Mahdian and Yan \cite{Mahdian2011}) and a $0.6534$ ratio (due to Huang et al. \cite{huang2018online}) for vertex weighted graphs. Thus, randomization does \AB{seem} to help in the classical ROM setting. 
%\ABc{I phrased this as "does seem to help" as I do not know of any negative results (beyond Mandshadi) that holds for deterministic algorithms and ROM inputs. We do know that randomization helps for adversarial inputs.} 


\end{itemize}



==> content/vertex_weights_proofs.tex <==
\begin{proof}[Proof of Theorem \ref{thm:efficient_star_dp}]
Recall that $G=(U,V,E)$ is a vertex-weighted stochastic graph
with substring-closed and permutation-closed probing constraints $(\scr{C}_v)_{v \in V}$.
It will also be convenient to denote $w_{u,s}:=w_{u}$ for each $u \in U$
such that $(u,s) \in \partial(s)$.

We first must show that there exists some $\bm{e}' \in \scr{C}_{s}$
such that $\val(\bm{e}') = \OPT(s,U)$, where 
\begin{equation}\label{eqn:expected_value_of_edge_probes}
	\val(\bm{e}):= \sum_{i=1}^{|\bm{e}|} p_{e_i} w_{e_i} \prod_{j=1}^{i-1} (1 - p_{e_i}),
\end{equation}
for $\bm{e} \in \scr{C}_s$, and $\OPT(s,U)$ is the value of the committal benchmark on $G[\{s\}\cup U]$.
Since the committal benchmark must respect commitment -- i.e., match the first
edge to $s$ which it reveals to be active -- it is clear that $\bm{e}'$ exists.


Let us now additionally assume that $\scr{C}_s$ is also closed under permutations.
Our goal is to show that $\bm{e}'$ can be computed efficiently.
Now, for any $\bm{e} \in \scr{C}_s$, let $\bm{e}^{r}$ be the rearrangement of $\bm{e}$, based on the non-increasing order
of the weights $(w_{e})_{e \in \bm{e}}$. Since $\scr{C}_s$ is closed under permutations,
we know that $\bm{e}^{r}$ is also in $\scr{C}_s$. Moreover, $\val(\bm{e}^{r}) \ge \val(\bm{e})$.
Hence, let us order the edges of $\partial(s)$ as $e_{1}, \ldots ,e_{m}$,
such that $w_{e_1} \ge \ldots \ge  w_{e_m}$, where $m:=|\partial(v)|$.
Observe then that it suffices to maximize \eqref{eqn:expected_value_of_edge_probes} over
those strings within $\scr{C}_s$ which respect this ordering on $\partial(s)$.
Stated differently, let us denote $\scr{I}_{s}$ as the family of subsets of $\partial(s)$
induced by $\scr{C}_s$, and define the set function $f: 2^{\partial(s)} \rightarrow [0, \infty)$,
where $f(B):= \val(\bm{b})$ for $B=\{b_{1}, \ldots ,b_{|B|}\} \subseteq \partial(s)$,
such that $\bm{b}=(b_{1}, \ldots ,b_{|B|})$ and $w_{b_1} \ge \ldots \ge w_{b_{|B|}}$.
Our goal is then to efficiently maximize $f$ over the set-system $(\partial(s),\scr{I}_s)$.
Observe that since $\scr{C}_s$ is both substring-closed and permutation-closed, 
$\scr{I}_s$ is downward closed. Moreover, clearly we can simulate oracle access to
$\scr{I}_s$, based on our oracle access to $\scr{C}_s$.


For each $i=0, \ldots ,m-1$, denote $\partial(v)^{>i}:=\{e_{i+1}, \ldots ,e_{m}\}$,
and $\partial(s)^{>m}:= \emptyset$. Moreover, define the family of subsets $\scr{I}_{s}^{>i}:= \{B \subseteq \partial(v)^{>i} : B \cup \{e_i\} \in \scr{I}_v\}$ for each $2 \le i \le m$, and $\scr{I}_{v}^{>0}:= \scr{I}_v$. Observe then that
$(\partial(v)^{>i}, \scr{I}_{v}^{>i})$ is a downward-closed set system, as $\scr{I}_v$ is downward-closed.
Moreover, we may simulate oracle access to $\scr{I}^{>i}_{v}$ based on our oracle access to $\scr{I}_v$.


Denote $\OPT(\scr{I}_{s}^{>i})$ as the maximum value of $f$ over constraints $\scr{I}_{s}^{>i}$.
Observe then the following recursion:
\begin{equation} \label{eqn:dynamical_program}
	\OPT(\scr{I}_{s}) :=  
			\max_{i \in [m]} ( p_{e_i} \cdot w_{e_i} + (1 - p_{e_i}) \cdot \OPT(\scr{I}_{s}^{>i}) )
\end{equation}
Hence, given access to the values $\OPT(\scr{I}_{s}^{>1}), \ldots , \OPT(\scr{I}_{s}^{>m})$,
we can compute $\OPT(\scr{I}_s)$ efficiently. In fact, it is clear that we can use \eqref{eqn:dynamical_program}
to recover an optimum solution to $f$, and so the proof follows by an inductive argument on $|\partial(s)|$.
We can define \textsc{DP-OPT} to be a memoization based implementation of \eqref{eqn:dynamical_program}.
\end{proof}


\begin{example} \label{example:bad_OPT_behaviour}
Let $G = (U, V, E)$ be a bipartite graph with $U = \{u_1, u_2, u_3, u_4\}$, $V = \{v\}$ and $\ell_v =2$. 
Set $p_{u_1, v} = 1/3$, $p_{u_2, v} = 1$, $p_{u_3, v} = 1/2$, $p_{u_4, v} = 2/3$.
Fix $\eps > 0$, and let the weights of offline vertices be $w_{u_1} = 1 + \eps$, $w_{u_2} = 1 + \eps/2$, $w_{u_3} = w_{u_4} = 1$. 
We assume that $\eps$ is sufficiently small -- concretely, $\eps \le 1/12$.
If $R_{1}:= U$, then $\OPT(v,R_1)$ probes $(u_{1},v)$ and then $(u_{2},v)$ in order. On the other hand,
if $R_{2} = R_{1} \setminus \{v_{2}\}$, then $\OPT(v,R_{2})$ does \textit{not} probe $(u_{1},v)$. Specifically,
$\OPT(v,R_{2})$ probes $(u_3,v)$ and then $(u_4,v)$.
\end{example}




\begin{proof}[Proof of Proposition \ref{prop:offline_dual_variable_lower_bound_general}]
For each $v \in V$, denote $R^{\text{af}}_{v}(G)$ as the unmatched (remaining) vertices of
$U$ right after $v$ is processed (attempts its probes) in the execution on $G$. We emphasize that if a probe of $v$
yields an active edge, thus matching $v$, then this match is excluded from $R^{\text{af}}_{v}(G)$.
Similarly, define $R^{\text{af}}_{v}(\til{G})$ in the same way for the execution on $\til{G}$
(where $v$ is now restricted to $\til{V}$).

Now, since $G$ is rankable and the constraints $(\scr{C}_v)_{v \in V}$ are substring-closed,
we can use the coupling between the two executions to inductively prove that
\begin{equation}\label{eqn:monotonicity_general}
	R^{\text{af}}_{v}(G) \subseteq R^{\text{af}}_{v}(\til{G}),
\end{equation}
for each $v \in \til{V}$ \footnote{Example \ref{example:bad_OPT_behaviour} shows why \eqref{eqn:monotonicity_general} will not hold if $G$ is not rankable.}. Now, since $g(1)=1$ (by assumption), there is nothing to prove if
$\til{Y}_{c}=1$. Thus, we may assume that $\til{Y}_c < 1$, and as a consequence,
that there exists some vertex $v_{c} \in V$ which matches to $u_0$ at time $\til{Y}_c$
in the execution on $\til{G}$.

On the other hand, by assumption we know that $u_0 \notin R^{\text{af}}_{v_c}(\til{G})$
and thus by \eqref{eqn:monotonicity_general}, that $u_0 \notin R^{\text{af}}_{v_c}(G)$.
As such, there exists some $v' \in V$ which probes $(u_0,v')$ and succeeds
in matching to $u_0$ at time $Y_{v'} \le \til{Y}_c$. Thus,
since $g$ is monotone,
\[
	\alpha_{u_0}  \ge \frac{w_{u_0}}{F} \, (1 - g(Y_{v'})) \, \bm{1}_{[ \til{Y}_c < 1]} \ge  \frac{w_{u_0}}{F} \, (1 - g(\til{Y}_c)),
\]
and so the claim holds.

\end{proof}


\begin{proof}[Proof of Lemma \ref{lem:dual_feasibility_constraints_general}]
We first observe that by taking the appropriate conditional expectation, 
Proposition \ref{prop:offline_dual_variable_lower_bound_general} ensures that
\[
	\mb{E}[\alpha_{u_0} \, | \, (Y_{v})_{v \in \til{V}}, (\sta(e))_{e \in \til{E}}] \ge \frac{w_{u_0}}{F} \cdot (1 - g(\til{Y}_c)),
\]
where the right-hand side follows since $\til{Y}_c$ is entirely determined from $(Y_{v})_{v \in \til{V}}$ and $(\sta(e))_{e \in \til{E}}$. Thus, combined with Proposition \ref{prop:online_dual_variable_lower_bound_general},
\[
	\mb{E}[ p_{u_0,v_0} \cdot \alpha_{u_0}+   w_{u_0} \cdot p_{u_0,v_0} \cdot \sum_{\substack{R \subseteq U: \\ u_0 \in R}} \phi_{v,R} \, | \, (Y_{v})_{v \in \til{V}}, (\sta(e))_{e \in \til{E}}],
\]
is lower bounded by
\[
	\frac{w_{u_0} \cdot p_{u_0,v_0}}{F} \cdot ( 1 - g( \til{Y}_c)) + \frac{w_{u_0} \, p_{u_0,v_0}}{F} \int_{0}^{\til{Y}_c} g(z) \, dz .
\]
However, $g(z):= \exp(z-1)$ for $z \in [0,1]$ by assumption, so
\[
	( 1 - g( \til{Y}_c)) + \int_{0}^{\til{Y}_c} g(z) \, dz = \left(1 - \frac{1}{e} \right),
\]
no matter the value of the critical time $\til{Y}_c$. As such, since $F:= 1 - 1/e$,
we may apply the law of iterated expectations and conclude that
\[
\mb{E}[p_{u_0,v_0} \cdot \alpha_{u_0} + w_{u_0} \cdot p_{u_0,v_0} \cdot \sum_{\substack{R \subseteq U: \\ u_0 \in R}} \phi_{v,R}] \ge w_{u_0} \cdot p_{u_0,v_0}.
\]
As the vertices $u_{0} \in U$ and $v_{0} \in V$ were chosen arbitrarily, the
proposed dual solution of Lemma \ref{lem:dual_feasibility_constraints_general} is feasible, 
and so the proof is complete.

\end{proof}

